The Risks, Benefits, and Consequences of Prepublication Moderation: Evidence from 17 Wikipedia Language Editions

Many online communities rely on postpublication moderation where contributors, even those that are perceived as being risky, are allowed to publish material immediately and where moderation takes place after the fact. An alternative arrangement involves moderating content before publication. A range of communities have argued against prepublication moderation by suggesting that it makes contributing less enjoyable for new members and that it will distract established community members with extra moderation work. We present an empirical analysis of the effects of a prepublication moderation system called FlaggedRevs that was deployed by several Wikipedia language editions. We used panel data from 17 large Wikipedia editions to test a series of hypotheses related to the effect of the system on activity levels and contribution quality. We found that the system was very effective at keeping low-quality contributions from ever becoming visible. Although there is some evidence that the system discouraged participation among users without accounts, our analysis suggests that the system's effects on contribution volume and quality were moderate at most. Our findings imply that concerns regarding the major negative effects of prepublication moderation systems on contribution quality and project productivity may be overstated.

==> full_review.tex <==
Dear Chau Tran    ,

Re: CSCW 2021 (April 2021 submissions) submission

     2781 - The risks, benefits, and consequences of pre-publication moderation: Evidence from 17 Wikipedia language editions

We are notifying you that your submission was recommended for Major Revision. The reviews can be found at the bottom of this email. Most papers received two external reviews plus a review from a 2AC and a meta-review from a 1AC. 

Please submit your revised submission plus a Summary of Revisions document by October 15, 2021 (midnight, AoE). You should submit your materials to the same form as your original submission (i.e., CSCW 2021 (April 2021 submissions) submissions). If you do not submit your revisions by October 15, your paper will be considered withdrawn. In that case, any resubmission of the work will be treated as a new submission and will be allocated new ACs and new reviewers in the future cycles.

Your paper is still in submission and must not be submitted elsewhere. It must remain anonymized. If you wish to formally withdraw the paper please email the CSCW 2021 Paper Chairs at your earliest convenience to do so.   

Next steps:

- You need to submit a revised submission accompanied by a Summary of Revisions document. Please submit two versions of the paper: one with highlighted changes (e.g. by using colored text) to facilitate re-review, and one “clean” version. Both should be anonymised. The Summary of Revisions should also be anonymised and should list the reviewers' comments and your responses, even for comments that did not lead to changes in the manuscript (in which case you might explain why you chose not to make certain suggested changes). The Summary of Revisions can be a set of bullet points, a table, or numbered points by which reviewers' comments are summarized along with your changes. This is not a rebuttal, but rather a description of changes made, or of reasons you could not or chose not to follow the reviewers' suggestions.

- Your anonymized paper will be re-reviewed by the same set of committee members and reviewers where possible. The decisions your paper can receive next are either “Accept with Minor Revision” or “Reject”. There is no second opportunity for Major Revision. Note that a Major Revision decision does not mean your paper will necessarily be accepted in the second round. It will undergo a second-round review, considering the original material plus changes that were made, and a new recommendation will be made to the Editors and Paper Chairs who will oversee final decisions.

- Through PCS, you will be able to communicate anonymously with your 1AC. You should use this channel if you need further clarification of any requirements the 1AC has listed in the meta-review.


Sincerely,
Shaowen Bardzell, Siân Lindley, Aleksandra Sarcevic, CSCW 2021 Paper Chairs

---

Reviews for CSCW 2021 (April 2021 submissions round) submission 2781:



----------------------------------------------------------------

1AC review

  Confidence

    Confident - I am knowledgeable in the area

  1AC Recommendation to Editors

    Major Revision

  1AC Meta-Review

    The reviewers agree that the paper has the potential to make a solid contribution
    to the moderation literature that is likely to be of interest to the CSCW
    community. However, the paper has some weaknesses that should be addressed before
    publication. I encourage the authors to carefully read all of the reviewers'
    comments and address all their concerns in a revision. I suggest that the authors
    pay special attention to two aspects:

    First, the authors should expand the introduction and background sections to
    clarify the motivation of their work and the impact of their findings. For
    example:

    - The reviews wondered about the generalizability of the findings to other peer-
    production systems. Do the findings depend on the specific characteristics of
    Wikipedia? Why is Wikipedia the best platform for this analysis?

    - The paper needs to provide a more clear motivation for the analysis of pre-
    publication moderation given that it is not very common. This discussion should
    draw on existing moderation literature, including literature from CSCW. - If the
    paper wants to make a theoretical contribution, a more thorough theoretical
    development of the hypotheses would be required.

    - While the paper shows that pre-publication moderation may not have a negative
    effect, the evidence that it has a positive effect is weak, which brings into
    question the usefulness of the system, relative to post-publication moderation.

    Second, some technical shortcomings need to be addressed. For example:

    - Some of the used statistical methods make assumptions about data. The authors
    should show that these assumptions are met or use a different statistical
    approach.

    - A lack of significance does not imply a lack of effect (which is what the
    authors appear to conclude). Focusing on the maximum effect sizes would be more
    convincing.

----------------------------------------------------------------

2AC review

  Confidence

    Confident - I am knowledgeable in the area

  Recommendation to 1AC

    Major Revision

  Review

    The paper is aimed at arguing the usefulness of pre-publication moderation of
    content published in peer-production systems. Using data from 17 Wikis, the paper
    attempts to show that the pre-pub moderation (PPM) called “FlaggedRevs” only
    minimally affects participation of some unregistered users, and so, the claim is
    that this can be safely deployed widely. The paper has a cleanly designed study.
    The analyses and the conclusions are straightforward.

    However, there are a few things the paper must sufficiently address for it to be a
    strong contribution to the CSCW community

    - The motivation for deploying PPMs is poorly written in the Introduction and
    Background sections. The paper tries to generalize to all peer-production
    communities while abruptly transitioning to the context of Wikipedia. As the paper
    closes, there is little discussion on how this is generalizable beyond Wikipedia.
    The paper does not sufficiently address other systems that already have
    implementations of PPM in place. The background as well as the discussion sections
    could be organized better and further strengthened.
    - A large number of tests are conducted but there is no mention of any correction
    for multiple simultaneous tests. Since the observed effect sizes are very small,
    the correction might lead to nothing being statistically significant.
    - While the paper tries to present evidence that PPM does not significantly
    affect, the argument in favor of deployment is rather weak toward the paper’s
    conclusion. Mostly, there is a discussion of why this has been unsuccessful within
    Wikipedia. The authors themselves state in the introduction that PPM does not
    measurably improve the quality of contributions of the wikis on which it is
    implemented. What, then, is the end goal of this analysis?
    - There is little discussion on how pre-publication moderation compares with post-
    publication moderation and which of the two is more beneficial to deploy.

    If there is a good contribution here, strengthening these sections could help show
    the true worth of it.

----------------------------------------------------------------

Reviewer 1 review

  Confidence

    Confident - I am knowledgeable in the area

  Recommendation to 1AC

    Major Revision

  Review

    This paper used an example of ‘FlaggedRevs’ applied on Wikipedia (Wiki) to study
    how pre-publication (pre-pub) moderation works and affects users’ future peer
    production actions from three dimensions, including affected, unaffected users,
    and the whole community. It also discussed whether newcomers are affected by such
    moderation. Overall, this paper took an interesting angle to study one phase/type
    of content moderation and constructed reasonable models to answer the hypothesis.
    The methods and model designs were clear to test the hypotheses. However, I did
    consider this paper lacking sufficient literature support and development in both
    literature review and discussion sections, missing contributions to the CSCW
    community, and needing a clear definition of models’ details. The first two
    concerns rendered me to suggest a major revision decision. In the following
    narratives, I discussed my concerns, followed by actionable suggestions.

    First, in the introduction section, I am confused about how logically and
    theoretically we should pay attention to the pre-pub moderation phase, indicating
    the motivation of this study. As the authors mentioned, many internet platforms
    utilize post-moderation, and few use pre-moderation. However, authors stood as
    human moderation’s angle to consider content moderation’s operational cost but did
    not clarify the motivation of exclusively focusing on such phase of moderation.
    Then, the authors also introduced controversies that exist on pre-pub moderation
    systems of Wiki, but what specific reason did authors focus on this a peer
    production site? I am also confused about why the authors put forward three
    questions, which are not research questions, in line 58 but did not answer at all
    (partially answered the third one). Thus, I recommend the authors clarify the
    motivation and background of why they want to focus on pre-pub moderation instead
    of post-pub or post-reactive moderation and choose Wiki as their study site (which
    could be also elaborated in the ‘empirical setting’ section). Also, the authors
    could clarify their research questions, meaning that how those four sets of
    hypotheses could be synthesized to answer what question of pre-pub moderation.

    Second, I felt the background section lacks literature support given the growing
    work around content moderation in the CSCW community. Specifically, on the one
    hand, at line 116, instead of focusing on introducing pre-pub moderation, the
    authors introduced several reasons for internet platforms utilizing post-pub
    moderation mode without any literature support. I am confused about the meaning of
    introducing advantages of post-pub moderation here, which is conflicted with the
    topic of this paper. It also rendered that the research gap (line 265) was not
    solid designed to tell us why we would care about pre-pub moderation’s impacts
    given it is applied on few platforms. So, I recommend authors clarify or adjust
    their phrasing or wording to stress the motivation/importance to study pre-pub
    moderation. On the other hand, the narratives, starting from line 116, are also
    without any literature support. Especially, given the statement that “it is
    relatively low-cost because not all content must be reviewed,” I somewhat disagree
    because many platforms use automated tools to consistently flag content, rendering
    it to moderators or directly making moderation decisions. Also, for the statement
    “The reactive nature of post-publication moderation systems means that malicious
    behaviors such as trolling, flaming and spamming can potentially go unnoticed and
    lead to low satisfaction among user (Butler, 1999),” with which I disagree because
    since now many automated moderation tools have been applied on internet platforms,
    abusive content is hard to be ignored, but may falsely be moderated, rendering
    those users’ lower satisfaction (Gorwa et al., 2020; Jhaver et al., 2019; Vaccaro
    et al., 2020). I thought the authors’ statement here happened at a much earlier
    time when there is only human moderation instead of human collaborating with
    automated moderation nowadays (Grimmelmann, 2015). Thus, I suggest the authors
    elaborate and clarify their literature review to clearly describe how pre-pub
    moderation works by citing more work from the CSCW and HCI communities since this
    version is now under-developed. In this way, I also recommend the authors could
    clarify why you choose ‘FlaggedRevs’ as the study site and how it works on Wiki
    more clearly. After reading the empirical setting section, I still cannot find how
    this tool makes moderation decisions either from established users, automated
    tools, or a mixture of both.

    Third, the main concerns for the model design are definitions of the measurements
    in the hypotheses. For example, in line 357, the authors defined their third
    hypothesis of the research methods by focusing on users’ contribution actions.
    However, it could be more precise, as the authors acknowledged, phrasing the
    hypothesis to focus on ‘contribution actions to the article page’ instead of
    simply indicating ‘contributions’ since this hypothesis did not intend to
    synthesize factors to analyze a category of user actions.

    Based on the results, I believed the discussion section was underdeveloped without
    connecting relevant literature in the CSCW and HCI community. Since this paper
    focused on how the impacts of those Wiki equipped with FlaggedRevs on users’
    contribution actions, it did not even elaborate such finding would connect and
    communicate with current literature of content moderation, nor implicate what can
    we learn from the findings to implicate pre-pub moderation mechanisms, or
    generally, considerations of using pre-pub mode in the general content moderation.
    I suggest the authors elaborate more on how your empirical findings could
    contribute to the literature, especially the growing body of ones discussing
    content moderation in the CSCW community.

    By the way, there were some small mistakes that needed the authors to scrutinize
    the paper’s phrasing. For example, in the abstract, it should be ‘our’ analysis
    instead of ‘out.’ Also, more than one mistake appeared in the hypotheses’ wording.

    Citations
    Gorwa, R., Binns, R., & Katzenbach, C. (2020). Algorithmic content moderation:
    Technical and political challenges in the automation of platform governance. Big
    Data & Society, 7(1), 205395171989794. https://urldefense.proofpoint.com/v2/url?u=https-3A__doi.org_10.1177_2053951719897945&d=DwIDaQ&c=slrrB7dE8n7gBJbeO0g-IQ&r=ZTlerZc-7XZuydWd1Spgrt0n-HhtiBfL1YPvvRzBmHI&m=bNDMQ_Q60M8gGcm2FdJX5l15DUWzHY9KSzAtZ1Rpuwo&s=648s24h89_iWzZlk5fdDdr8acwTaAy06-bkqxprMM_Y&e=
    Grimmelmann, J. (2015). The Virtues of Moderation. Yale Journal of Law and
    Technology, 17. https://urldefense.proofpoint.com/v2/url?u=https-3A__heinonline.org_HOL_Page-3Fhandle-3Dhein.journals_yjolt17-26id-3D42&d=DwIDaQ&c=slrrB7dE8n7gBJbeO0g-IQ&r=ZTlerZc-7XZuydWd1Spgrt0n-HhtiBfL1YPvvRzBmHI&m=bNDMQ_Q60M8gGcm2FdJX5l15DUWzHY9KSzAtZ1Rpuwo&s=yBN8JPgyqYEHAem4BQcXxraIuaLzg05KMRKI7unFYL0&e=
    &div=&collection=
    Jhaver, S., Appling, D. S., Gilbert, E., & Bruckman, A. (2019). “Did you suspect
    the post would be removed?”: Understanding user reactions to content removals on
    reddit. Proceedings of the ACM on Human-Computer Interaction, 3(CSCW), 1–33.
    https://urldefense.proofpoint.com/v2/url?u=https-3A__doi.org_10.1145_3359294&d=DwIDaQ&c=slrrB7dE8n7gBJbeO0g-IQ&r=ZTlerZc-7XZuydWd1Spgrt0n-HhtiBfL1YPvvRzBmHI&m=bNDMQ_Q60M8gGcm2FdJX5l15DUWzHY9KSzAtZ1Rpuwo&s=iz9Jeu2_KV7Dceb5bPw3GDiKIhLwUnlEfqOuJYchbRw&e=
    Vaccaro, K., Sandvig, C., & Karahalios, K. (2020). “At the End of the Day Facebook
    Does What It Wants”: How Users Experience Contesting Algorithmic Content
    Moderation. Proceedings of the ACM on Human-Computer Interaction, 4(CSCW2), 1–22.
    https://urldefense.proofpoint.com/v2/url?u=https-3A__doi.org_10.1145_3415238&d=DwIDaQ&c=slrrB7dE8n7gBJbeO0g-IQ&r=ZTlerZc-7XZuydWd1Spgrt0n-HhtiBfL1YPvvRzBmHI&m=bNDMQ_Q60M8gGcm2FdJX5l15DUWzHY9KSzAtZ1Rpuwo&s=_sJb5EeGq8eySgXG1g1l6Knc77tgMhFqPXgYUpIDzQE&e=

----------------------------------------------------------------

Reviewer 3 review

  Confidence

    Confident - I am knowledgeable in the area

  Recommendation to 1AC

    Major Revision

  Review

    The paper evaluates the effect of a pre-publication moderation system in 17
    Wikipedia language communities, with attention to the quality of submissions and
    productivity of editors. Authors apply Interrupted Time Series analysis and a
    general linear model to address these questions. The authors conclude that pre-
    publication moderation can be an effective way to reduce the number of low-quality
    submissions among some groups of editors, with little observed reduction in the
    overall productivity of editors.

    Overall, this paper is clear and well-writen, and addresses a potentially high-
    impact topic. However, some important details are missing from the model and
    methods. The discussion is somewhat limited and would benefit from expansion. I am
    recommending a major revision because I cannot know if the paper's results will
    hold true after my concerns are addressed, but if they do, I believe the
    contribution presented in this paper will make a valuable contribution to the CSCW
    literature.

    The question addressed by this paper applies to most forms of peer production,
    with varying levels of impact. While vandalism on Wikipedia is a nuisance, it has
    typically been found to be reliably corrected in time. On the other hand, both
    targeted misinformation and malicious changes to free/open-source software can
    have significant impact. Many studies, as acknowledged by the authors, have found
    higher barriers to entry to be detrimental to peer production communities, so
    moderation systems not displaying this detrimental behavior are potentially high
    impact. The paper is limited to a single platform (Wikipedia), although the scale
    of Wikipedia and the breadth of community norms across language editions are a
    strength of the paper. The methods are conceptually straightforward, but non-
    trivial to apply at the scale of Wikipedia.

    The use of ITS and GLMM for wiki-level and user-level analyses seem appropriate.
    It is not clear whether the dependent variables were tested to verify the
    necessary conditions for linear regression. In particular, heavy-tailed
    distributions can lead to non-normally-distributed residuals. Otherwise, the
    analysis appears well-executed, and results are clearly stated both visually and
    in table form.

    The paper is well-writen, and the methods clearly communicated. The background
    focuses on mostly on Wikipedia-related literature and the paper would benefit from
    drawing clearer distinctions between Wikipedia, peer production in genera, and
    content moderation in general, as well as expanding explanations of how this work
    fits into (or not) each of those contexts. As the findings of the paper might seem
    counter to conclusions of some of the literature, the paper would benefit from an
    expanded discussion of how these findings can be reconciled.

    While this is a strong paper, there are a few potential weaknesses that could be
    addressed. The potentially limited generalizability is worth discussing. The
    potential inclusion of both affected and non-affected users in the returning
    editor group is a potentially serious issue, although it does not seem to
    undermine the key findings. Similarly, the lack of significance is presented as
    evidence of a lack of an effect, which is theoretically questionable. This issue
    could be addressed by providing a bound on the effect size in cases when the
    observed effect does not meet the significance threshold. One final issue is the
    claim in the introduction that a theoretical contribution is made. The paper does
    not seem to develop or propose theoretical contributions, although the other
    contributions should be sufficient.

    Suggested Changes:
    * All independent variables for the regressions, including controls, should be
    listed. Although it is reasonable to omit regression results for controls.
    * Normality of residuals should be confirmed for linear regressions.
    * Theoretical contribution should be expanded, or removed as a claimed
    contribution.
    * Expand discussion of how findings can be reconciled with previous literature.

    Minor Notes:
    * The casual use of the phrase "collateral damage" is potentially insensitive.
    * It would be interesting to further explore the discrepancy between IP users and
    first-time registered users. Do the decreases in reverts correspond to a higher
    number of quality submissions or a lower number of low-quality submissions, or
    both?

----------------------------------------------------------------



End of reviews for CSCW 2021 (April 2021 submissions round) submission 2781
